Self-Supervised Learning for Endoscopic Video Analysis

Self-supervised learning (SSL) has led to important breakthroughs in computer vision by allowing learning from large amounts of unlabeled data. As such, it might have a pivotal role to play in biomedicine where annotating data requires a highly specialized expertise. Yet, there are many healthcare domains for which SSL has not been extensively explored. One such domain is endoscopy, minimally invasive procedures which are commonly used to detect and treat infections, chronic inflammatory diseases or cancer. In this work, we study the use of a leading SSL framework, namely Masked Siamese Networks (MSNs), for endoscopic video analysis such as colonoscopy and laparoscopy. To fully exploit the power of SSL, we create sizable unlabeled endoscopic video datasets for training MSNs. These strong image representations serve as a foundation for secondary training with limited annotated datasets, resulting in state-of-the-art performance in endoscopic benchmarks like surgical phase recognition during laparoscopy and colonoscopic polyp characterization. Additionally, we achieve a 50% reduction in annotated data size without sacrificing performance. Thus, our work provides evidence that SSL can dramatically reduce the need of annotated data in endoscopy.

==> sections/acknowledgment.tex <==
% \paragraph{\textbf{Data Use Declaration}}
% \subsection*{Data Use Declaration and Acknowledgment:}
% \todo{Authors must declare the data origin, data license, and (when appropriate) ethics application number for any public or private data used in the preparation of the paper. The paper must include the co-authors, paper citations, and/or acknowledgments as required by any public or private data used in the preparation of the paper. The data use declaration and acknowledgment must be properly anonymized for the double-blind review process.}
% \todo{IRB approval was granted prior to commencing the study.}
